SoCal: A Language for Memory-Layout Factorization of Recursive Datatypes

Array-of-structures (AoS) to structure-of-arrays (SoA) is a classic compiler transformation that improves memory locality and enables data-parallel execution. Existing AoS-to-SoA transformations target regular, array-based programs in imperative languages, such as C. However, many applications traverse tree-shaped data such as ASTs in compilers, DOM trees in browsers, and k-d trees in scientific workloads. Prior work speeds up functional programs over trees by serializing algebraic datatypes (ADTs) into one contiguous buffer. Such a representation interleaves the fields of every node, similar to an AoS layout. We introduce a factored layout of ADTs, which stores its fields in separate buffers, producing a layout that resembles SoA. In a factored layout, a traversal can focus on relevant fields and ignore the rest, similar to extracting a column from a SoA representation; in this setting, traversals over scalar fields can be vectorized. Working with raw byte arrays is error-prone, though: wrong indexing can silently read bytes from a wrong field or write past the end of a value. We therefore introduce SoCal, a type-safe language for expressing traversals over factored ADTs. Our compiler, Colobus, transforms a simple functional language with ADTs reminiscent of Haskell to C, using SoCal as the intermediate representation. Colobus generates traversals over byte arrays in the factored representation and performs optimizations such as field skipping and vectorization. Across a suite of benchmarks, Colobus shows the average speedups of 3.8x and 5.2x over fold and map passes, respectively.

==> editingmarks.tex <==


\usepackage{todonotes}

\newcommand{\rn}[1]{\pgwrapper{RRN}{#1}}  %

\newcommand{\tlm}[1]{\pgwrapper{TLM}{#1}} %
\newcommand{\bjs}[1]{\pgwrapper{BJS}{#1}} %
\newcommand{\chc}[1]{\pgwrapper{CHC}{#1}} %
\newcommand{\vc}[1]{\pgwrapper{VC}{#1}} %
\newcommand{\bc}[1]{\pgwrapper{BC}{#1}} %
\newcommand{\mv}[1]{\pgwrapper{MV}{#1}} %
\newcommand{\osa}[1]{\pgwrapper{OSA}{#1}} %
\newcommand{\mm}[1]{\pgwrapper{MM}{#1}} %
\newcommand{\rgs}[1]{\pgwrapper{RGS}{#1}} %
\newcommand{\csk}[1]{\pgwrapper{CSK}{#1}} %

\newcommand{\mk}[1]{\pgwrapper{MK}{#1}} %
\newcommand{\ls}[1]{\pgwrapper{LS}{#1}} %
\newcommand{\vs}[1]{\pgwrapper{VS}{#1}} %
\newcommand{\ap}[1]{\pgwrapper{AP}{#1} } %

\newcommand{\spall}[1]{\pgwrapper{SS}{#1}} %

\newcommand{\jd}[1]{\pgwrapper{JD}{#1}} %
\newcommand{\onl}[1]{\pgwrapper{ONL}{#1}} %

\newcommand{\mr}[1]{\pgwrapper{MR}{#1}} %
\newcommand{\mtk}[1]{\pgwrapper{MTK}{#1}} %


\InputIfFileExists{activateeditingmarks}{
}{
    \def\noeditingmarks{}
}

\definecolor{comment-red}{rgb}{0.8,0,0}
\definecolor{dark-green}{rgb}{0.0,0.4,0}
\definecolor{dark-blue}{rgb}{0.0,0.0,0.55}
\definecolor{very-dark-green}{rgb}{0.0,0.3,0}

\ifx\noeditingmarks\undefined
   \newcommand{\auditme}[1]{{\color{dark-green}{#1}}}

   \newcommand{\fixme}[1]{{\color{comment-red}{#1}}}

   \newcommand{\note}[1]{{\begin{itemize}\item \textcolor{blue}{NOTE: #1} \end{itemize}}}

   \newcommand{\new}[1]{{\color{blue}{#1}}}

   \newcommand{\const}[1]{\textred{#1}}
   \definecolor{mygrey}{rgb}{0.7,0.7,0.7}

   \newcommand{\textred}[1]{{\color{comment-red}{#1}}}

   \makeatletter\@mparswitchfalse\makeatother
   \normalmarginpar
   \setlength{\marginparsep}{3pt}
   \setlength{\marginparwidth}{\dimexpr(\paperwidth-\textwidth)/2-\marginparsep-4pt\relax}
   \DeclareRobustCommand{\pgwrapperinline}[2]{%
     \ifmmode
       \mbox{\textcolor{comment-red}{[#1: #2]}}%
     \else
       {\textcolor{comment-red}{[#1: #2]}}%
     \fi
   }
   \DeclareRobustCommand{\pgwrapper}[2]{%
     \ifmmode
       \pgwrapperinline{#1}{#2}%
     \else
       \ifinner
         \pgwrapperinline{#1}{#2}%
       \else
         \todo[size=\scriptsize]{#1: #2}%
       \fi
     \fi
   }

   \InputIfFileExists{activategreybg}{
       \definecolor{comment-red}{rgb}{0.5,0,0}
       \pagecolor{mygrey}
   }{}

  \newcommand{\rnfloat}[1]{\pgwrapper{RRN}{#1}\vspace{-4mm}}  %

\else
   \newcommand{\textred}[1]{{\color{comment-red}{#1}}}
   \newcommand{\auditme}[1]{#1}
   \newcommand{\fixme}[1]{\textred{#1}}
   \newcommand{\pgwrapper}[2]{}
   \newcommand{\note}[1]{{\begin{itemize}\item {\textcolor{blue}{#1}} \end{itemize}}}
   \newcommand{\new}[1]{{\color{blue}{#1}}}
   \newcommand{\const}[1]{#1}

   \newcommand{\rnfloat}[1]{}  %
\fi

\newcommand{\Red}[1]{\textred{#1}}

\newcommand{\ie}{{i.e.,}}
\newcommand{\eg}{{e.g.,}}
\newcommand{\etal}{\textit{et al.}}

\def\scrunchit{}
\ifx\scrunchit\undefined
  \newcommand{\captionscrunch}{}
\else
  \newcommand{\captionscrunch}{\vspace{-3mm}}
\fi

\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\Secref}[1]{\secref{#1}}

\newcommand{\Figref}[1]{Figure~\ref{#1}}
\newcommand{\figref}[1]{\Figref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}


\newcommand{\appendixref}[1]{\ref{#1}}
\newcommand{\Appendixref}[1]{\ref{#1}}


==> formal_grammar_aux.tex <==
\begingroup
\setlength{\arraycolsep}{1pt}
\renewcommand{\arraystretch}{1.08}

\formalcontentblock{\footnotesize
  \formalgrammarkeywords
  \socalgrammardisplays
  \socalgrammargrid{\textup{Location Expressions}}{\mathit{pat}}%
  \socalgrammarhead{Terms}%
  \input{paper-formalism/paper-fragments/gr-termgrammar}%
  \input{paper-formalism/paper-fragments/gr-locexpr}%
  \par\vspace{\socalgrammargap}%
  \socalgrammarhead{Run-time state}%
  \[
    \begin{array}{G}
      \textup{Layout Cursor} & c & \gramdef &
        \ngCurs{i}\,\overharpoon{(\DC,\,j,\,c_{\DC,j})}
    \end{array}
  \]
  \[
    \begin{array}{G}
      \textup{Location Map} & \MENV & \gramdef & \set{\ngLoc_1^{\ngPos_1} \mapsto c_1, \ldots}
    \end{array}
  \]
  \[
    \begin{array}{G}
      \textup{Write Event} & w & \gramdef & (\ngCell{\ngPos}{i},\DC) \\
      \textup{Store} & \STOR & \gramdef & \varepsilon \gramor \STOR \cdot w
    \end{array}
  \]
}

\endgroup


==> formal_grammar_core.tex <==
\begingroup
\setlength{\arraycolsep}{1pt}
\renewcommand{\arraystretch}{1.08}

\formalcontentblock{\footnotesize
  \formalgrammarkeywords
  \socalgrammardisplays
  \socalgrammargrid{\textup{Datatype Declarations}}{\mathit{top}}%
  \socalgrammarhead{Programs, types and locations}%
  \input{paper-formalism/paper-fragments/gr-program-top}%
  \input{paper-formalism/paper-fragments/gr-datadecl}%
  \input{paper-formalism/paper-fragments/gr-locatedtypes-scheme}%
  \input{paper-formalism/paper-fragments/gr-functiondecl}%
  \input{paper-formalism/paper-fragments/gr-paths-positions}%
  {\socalgrammargrid{}{\SENV,\NENV,\UENV}%
   \socalgrammarhead{Typing environments}%
   \input{paper-formalism/paper-fragments/gr-env-core}%
   \input{paper-formalism/paper-fragments/gr-env-regiontyped}%
   \[
     \begin{array}{H}
       \ngAP & \gramdef & \phi \gramor \ngFam \\
       \ngFam & \gramdef & \set{\ngPath_1 \mapsto \ngLoc_1, \ldots}
     \end{array}
   \]
  }%
}

\endgroup


==> haskell_style.tex <==

\usepackage{upquote}
\usepackage{listings}
\usepackage{iftex}
\usepackage[]{xcolor}
\definecolor{MidnightBlue}{rgb}{0.1, 0.1, 0.44}

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkred}{rgb}{0.5,0,0}
\definecolor{hsbg}{HTML}{FFFFFF}
\definecolor{hsbgblock}{HTML}{FFFFFF}
\definecolor{hsfg}{HTML}{000000}
\definecolor{hskw}{HTML}{0000FF}
\definecolor{hstype}{HTML}{0000FF}
\definecolor{hsctor}{HTML}{000000}
\definecolor{hsfunc}{HTML}{000000}
\definecolor{hsop}{HTML}{000000}
\definecolor{hsstring}{HTML}{000000}
\definecolor{hscomment}{HTML}{5F6B7A}
\colorlet{cfg}{hsfg}
\colorlet{ckw}{hskw}
\colorlet{ctype}{hstype}
\colorlet{cfunc}{hsfg}
\colorlet{cmacro}{hskw}
\colorlet{cstring}{hsfg}
\colorlet{ccomment}{hscomment}

\lstset{%
    frame=none,
    backgroundcolor=\color{hsbg},
    rulecolor={\color{black}},
    numbers=none,
    basicstyle=\footnotesize\ttfamily\color{hsfg},
    numberstyle=\color{black!55}\tiny\itshape,
    commentstyle=\color{hscomment},
    stringstyle=\color{hsstring},
    keywordstyle=[1]\color{hskw},
    keywordstyle=[2]\color{hstype},
    keywordstyle=[3]\color{hsctor},
    keywordstyle=[4]\color{hsfunc},
    captionpos=b,
    aboveskip=1\medskipamount,
    xleftmargin=0.5\parindent,
    xrightmargin=0.5\parindent,
    flexiblecolumns=false,
    escapechar={\@},
    mathescape=true,
    texcl=true,                          %
    showstringspaces=false
}

\lstloadlanguages{Haskell}
\lstdefinestyle{haskell}{%
    language=Haskell,
    upquote=true,
    deletekeywords={case,class,data,default,deriving,do,in,instance,let,of,type,where,if,then,else,module,import,qualified,as,hiding,Int,Integer,Float,Double,Char,String,Bool,IO,ST,STM,Monad,List,Tree,Maybe,Either},
    morekeywords={[1]case,of,let,in,where,data,type,class,instance,deriving,do,if,then,else,module,import,qualified,as,hiding,letpacked,letloc,letreg,letregion,for,beyond},
    morekeywords={[2]Int,Integer,Float,Double,Char,String,Bool,IO,ST,STM,Monad,List,Tree,Maybe,Either,Cursor,CursorArray,MutCursor,Tag,Ptr,Region,RetProd},
    morekeywords={[3]Cons,Nil,Node,Leaf,Just,Nothing,True,False,Left,Right,Unbounded,Bounded},
    morekeywords={[4]map,foldr,foldl,filter,sumTree,add1Tree,buildtree,myFunc,advanceTags,advanceField,introLocVec,mkSoAReg,projTagLoc,projFieldLoc,start,after,readInt,writeInt,readTag,writeTag,readCursor,writeCursor,makeCursorArray,indexCursorArray,writeCursorMutable,addrOfCursor,derefMutCursor,bumpMutableCursor},
    literate=
        {\\}{{{\color{hsop}$\lambda$}}}1
        {Lambda}{{{\color{hsop}$\Lambda$}}}1
        {\\\\}{{\char`\\\char`\\}}1
        {>->}{{{\color{hsop}>->}}}3
        {>>=}{{{\color{hsop}>>=}}}3
        {->}{{{\color{hsop}$\rightarrow$}}}2
        {>=}{{{\color{hsop}$\geq$}}}2
        {<-}{{{\color{hsop}$\leftarrow$}}}2
        {<=}{{{\color{hsop}$\leq$}}}2
        {=>}{{{\color{hsop}$\Rightarrow$}}}2
        {::}{{{\color{hsop}::}}}2
        {<$>}{{{\color{hsop}<\$>}}}3
        {|}{{{\color{hsop}$\mid$}}}1
        {forall}{{{\color{hsop}$\forall$}}}1
        {exists}{{{\color{hsop}$\exists$}}}1
        {...}{{$\cdots$}}3
}

\lstdefinestyle{haskellblock}{%
    style=haskell,
    frame=none,
    backgroundcolor=\color{hsbgblock},
    xleftmargin=4mm,
    xrightmargin=0pt,
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    breakatwhitespace=true,
    aboveskip=1pt,
    belowskip=1pt
}

\definecolor{vsln}{HTML}{600000}   %
\newsavebox{\vscodepane}
\lstdefinestyle{vscodeblock}{%
    style=haskellblock,
    backgroundcolor={},
    numbers=left,
    numbersep=1.5mm,
    numberstyle=\color{vsln}\scriptsize\ttfamily
}

\lstdefinestyle{localblock}{%
    style=haskell,
    frame=none,
    backgroundcolor=\color{hsbgblock},
    basicstyle=\ttfamily\scriptsize\color{hsfg},
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    breakatwhitespace=false,
    resetmargins=true,
    linewidth=\columnwidth,
    xleftmargin=4mm,
    xrightmargin=0pt,
    aboveskip=0.4\baselineskip,
    belowskip=0.4\baselineskip,
    escapeinside={(*@}{@*)}
}

\lstdefinestyle{localtable}{%
    style=haskell,
    frame=none,
    backgroundcolor=\color{hsbg},
    basicstyle=\ttfamily\footnotesize\color{hsfg},
    columns=fullflexible,
    linewidth=\linewidth,
    breaklines=true,
    breakatwhitespace=false,
    resetmargins=true,
    xleftmargin=0pt,
    xrightmargin=0pt,
    aboveskip=0pt,
    belowskip=0pt,
    showstringspaces=false,
    escapeinside={(*@}{@*)}
}

\lstdefinestyle{cblock}{%
    basicstyle=\ttfamily\scriptsize\color{cfg},
    backgroundcolor=\color{hsbgblock},
    identifierstyle=\color{cfg},
    keywordstyle=[1]\color{ckw},
    keywordstyle=[2]\color{ctype},
    commentstyle=\color{ccomment},
    stringstyle=\color{cstring},
    showstringspaces=false,
    keepspaces=true,
    upquote=true,
    alsoletter={0123456789xABCDEFabcdef_},
    tabsize=2,
    columns=fullflexible,
    breaklines=true,
    breakatwhitespace=true,
    frame=none,
    xleftmargin=4mm,
    xrightmargin=0pt,
    aboveskip=1pt,
    belowskip=1pt,
    morecomment=[l][\color{cmacro}]{\#},
    deletekeywords={int,char,size_t,struct,float,double,void,bool,short,long,unsigned,signed,const,static,typedef,enum,uint8_t,uint16_t,uint32_t,uint64_t,int8_t,int16_t,int32_t,int64_t},
    morekeywords={[1]if,else,return,for,while,do,switch,case,break,continue,goto},
    morekeywords={[2]int,char,size_t,struct,float,double,void,bool,short,long,unsigned,signed,const,static,typedef,enum,uint8_t,uint16_t,uint32_t,uint64_t,int8_t,int16_t,int32_t,int64_t,byte,Cursor,RetProd,ptrset,footer},
    emph=[1]{printf,malloc,free,sumTree,add1Tree,sumPacked,my_func},
    emphstyle=[1]\color{cfunc},
    emph=[2]{NULL,true,false,LEAF_TAG, NODE_TAG, LEAF,INTERNAL,EOC,0xFF},
    emphstyle=[2]\color{ctype}\bfseries
}

\lstdefinestyle{inline}{%
    style=haskell,
    basicstyle=\footnotesize\ttfamily\color{hsfg},
    columns=fixed,
    basewidth=0.48em,
    keepspaces=false,
    breaklines=true,
    breakatwhitespace=true,
    escapechar={\@},
    mathescape=true,
    literate=
        {\\}{{{\color{hsop}$\lambda$}}}1
        {Lambda}{{{\color{hsop}$\Lambda$}}}1
        {\\\\}{{\char`\\\char`\\}}1
        {>->}{{{\color{hsop}>->}}}3
        {>>=}{{{\color{hsop}>>=}}}3
        {->}{{{\color{hsop}$\rightarrow$\space}}}3    %
        {>=}{{{\color{hsop}$\geq$}}}2
        {<-}{{{\color{hsop}$\leftarrow$}}}2
        {<=}{{{\color{hsop}$\leq$}}}2
        {=>}{{{\color{hsop}$\Rightarrow$}}}2
        {::}{{{\color{hsop}::}}}2
        {<$>}{{{\color{hsop}<\$>}}}3
        {|}{{{\color{hsop}$\mid$}}}1
        {forall}{{{\color{hsop}$\forall$}}}1
        {exists}{{{\color{hsop}$\exists$}}}1
        {...}{{$\cdots$}}3
}

\lstnewenvironment{code}
    {\lstset{style=haskellblock}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    {}

\lstset{style=haskell}

\newcommand{\il}[1]{\lstinline[style=inline,mathescape=true];#1;}
\newcommand{\lstinlineLOCAL}[1]{\lstinline[style=inline,basicstyle=\ttfamily\scriptsize\color{hsfg},columns=fullflexible,breaklines=true,breakatwhitespace=false,mathescape=true];#1;}
\newcommand{\cil}[1]{{\footnotesize\textcolor{ctype}{\texttt{#1}}}}
\newcommand{\cff}[1]{{\footnotesize\textcolor{cfunc}{\texttt{#1}}}}

\newcommand{\makeatcode}{\lstMakeShortInline[style=inline]@}
\newcommand{\makeatchar}{\lstDeleteShortInline@}


==> macros.tex <==



\let\overharpoon\relax
\makeatletter
\newcommand*\colobus@rightharpoonfill@{%
  \arrowfill@\relbar\relbar\rightharpoonup
}
\newcommand*\colobus@overrightharpoon{%
  \mathpalette{\overarrow@\colobus@rightharpoonfill@}%
}
\newcommand{\overharpoon}[1]{\colobus@overrightharpoon{#1}}
\makeatother




\makeatletter
\let\th@plain\relax
\makeatother
\usepackage[thmmarks,amsmath]{ntheorem}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}

\theorempreskip{0pt}
\theorempostskip{10pt}
\theoremheaderfont{\scshape}
\theorembodyfont{\upshape}
\theoremindent10pt
\newtheorem*{goal}{Obl.}

\theoremindent10pt
\newtheorem{subcase}{SubCase}
\theorempostwork{\setcounter{subcase}{0}}
\newtheorem{ncase}{Case}
\newtheorem*{bcase}{Case}

\theoremstyle{nonumberplain}
\theorempreskip{0pt}
\theorempostskip{10pt}
\theoremheaderfont{\scshape}
\theorembodyfont{\upshape}

\theorempostwork{\setcounter{ncase}{0}}
\newtheorem{proofsketch}{Proof Sketch}
\AtBeginEnvironment{proofsketch}{\color{red}}

\theorempostwork{\setcounter{ncase}{0}}
\newtheorem{nproof}{Proof}

\theoremstyle{plain}
\theorempreskip{6pt}
\theorempostskip{6pt}
\theoremindent0pt
\theoremheaderfont{\normalfont\bfseries}
\theorembodyfont{\normalfont}
\theoremsymbol{}
\let\definition\relax
\let\enddefinition\relax
\newtheorem{definition}{Definition}[section]



\input{editingmarks}

\input{haskell_style}

\input{paper-formalism/formalism-macros/defs.tex}

\input{paper-formalism/formalism-macros/socal-macros}

\newcommand{\socalprosekw}[1]{{\footnotesize\ttfamily\color{hskw}#1}}
\renewcommand{\gramkw}[1]{\relax\ifmmode\mathord{\text{\socalprosekw{#1}}}\else\socalprosekw{#1}\fi}
\renewcommand{\ctors}[1]{\mathrm{Ctors}(#1)}
\renewcommand{\typeoffield}{\mathrm{TypeOfField}}
\renewcommand{\fresh}{\mathrm{fresh}}


\renewcommand{\ngUnstarted}{\ensuremath{\phi}}
\renewcommand{\ngStarted}[1]{\ensuremath{#1}}

\providecommand{\ngRuleName}[1]{\textup{\textsc{#1}}}
\newcommand{\ngCfgWF}[4]{\mathrm{CfgWF}_{#1}(#2;#3;#4)}
\newcommand{\ngStepstoStar}{\;\ngRedArrow^*\;}
\newcommand{\ngPendUp}[3]{\ensuremath{\mathrm{PendingAfter}(#1;#2;#3)}}
\newcommand{\ngFocus}[1]{\mathrm{focus}(#1)}

\newcommand{\formalgrammarkeywords}{%
  \renewcommand{\gramkw}[1]{\mathord{\mathrm{##1}}}%
}


\definecolor{FormalText}{HTML}{000000}
\definecolor{FormalAccent}{HTML}{000000}
\definecolor{FormalBorder}{HTML}{C0C0C0}
\definecolor{FormalBg}{HTML}{FFFFFF}
\definecolor{FormalBgAlt}{HTML}{FFFFFF}
\definecolor{FormalMutedRow}{HTML}{E8E8E8}
\definecolor{FormalCodeKw}{HTML}{0000FF}

\newlength{\formalcolumnsep}
\setlength{\formalcolumnsep}{1.1em}

\newcolumntype{Y}{>{\raggedright\arraybackslash}X}

\newcommand{\formalseriffont}{}
\newcommand{\formalmonofont}{\fontfamily{zi4}\fontseries{m}\fontshape{n}\selectfont}
\newcommand{\formalcontentfont}{\footnotesize\formalseriffont}
\newcommand{\formalrulefont}{\fontsize{8}{9.4}\selectfont\formalseriffont}
\let\formalbasevdash\vdash
\newcommand{\formalkeyword}[1]{%
  \ifmmode
    \mathord{\mathrm{#1}}%
  \else
    \textup{#1}%
  \fi
}
\newcommand{\formalnonterminal}[1]{%
  \ifmmode
    \mathsf{#1}%
  \else
    \textsf{#1}%
  \fi
}
\newcommand{\formaltypename}[1]{%
  \ifmmode
    \mathsf{#1}%
  \else
    \textsf{#1}%
  \fi
}
\newcommand{\formalmetaid}[1]{%
  \ifmmode
    \mathit{#1}%
  \else
    \textit{#1}%
  \fi
}
\newcommand{\formaljudgesym}{\mathrel{\formalbasevdash}}
\newcommand{\formalstepsym}{\mathrel{\;\hookrightarrow\;}}
\newcommand{\formalclausesym}{\mathrel{\Rightarrow}}
\newcommand{\formalgrayrow}{\rowcolor{FormalMutedRow}}

\newcommand{\marmosetlang}[0]{\ensuremath{\lambda_{M}}}

\newcommand{\formalrulelabel}[1]{%
  \text{\formalseriffont\scshape [#1]}%
}
\newcommand{\formalgrayboxed}[2][0.2ex]{%
  \begingroup
  \let\color\socalkeepcolor
  \setlength{\fboxsep}{#1}%
  \mathchoice
    {\colorbox{FormalMutedRow}{$\displaystyle #2$}}%
    {\colorbox{FormalMutedRow}{$\textstyle #2$}}%
    {\colorbox{FormalMutedRow}{$\scriptstyle #2$}}%
    {\colorbox{FormalMutedRow}{$\scriptscriptstyle #2$}}%
  \endgroup
}
\setlength{\textfloatsep}{7pt plus 1pt minus 2pt}
\setlength{\floatsep}{5pt plus 1pt minus 2pt}
\setlength{\intextsep}{5pt plus 1pt minus 2pt}
\setlength{\dbltextfloatsep}{7pt plus 1pt minus 2pt}
\setlength{\dblfloatsep}{5pt plus 1pt minus 2pt}
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{1pt}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{8}
\setcounter{dbltopnumber}{2}
\renewcommand{\topfraction}{0.95}
\renewcommand{\dbltopfraction}{0.95}
\renewcommand{\bottomfraction}{0.90}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.85}
\renewcommand{\dblfloatpagefraction}{0.85}
\newcommand{\formalgraymath}[1]{%
  \formalgrayboxed[0.2ex]{#1}%
}
\newcommand{\formalgrayrule}[1]{%
  \formalgrayboxed[0.45ex]{#1}%
}

\newcommand{\formalcontentsymbols}{%
  \renewcommand{\gramkw}[1]{\formalkeyword{##1}}%
  \renewcommand{\gramwd}[1]{\gramkw{##1}}%
  \renewcommand{\sgramwd}[1]{\gramkw{##1}}%
  \renewcommand{\gramdef}{\;\mathrel{\coloneqq}\;}%
  \renewcommand{\gramor}{\;\mathrel{\mid}\;}%
  \renewcommand{\ARROW}{\mathrel{\rightarrow}}%
  \renewcommand{\caseclause}[2]{##1\;\formalclausesym\;##2}%
}

\newcommand{\formalsymbols}{%
  \formalcontentsymbols
  \renewcommand{\vdash}{\formaljudgesym}%
  \renewcommand{\stepsto}{\formalstepsym}%
}

\newcommand{\formalpaneltitle}[1]{%
  {\color{FormalText}\sffamily\bfseries\footnotesize\MakeUppercase{#1}}\par
  \vspace{2pt}%
  {\color{FormalAccent}\rule{\linewidth}{0.7pt}}\par
  \vspace{5pt}%
}

\let\socalkeepcolor\color
\newcommand{\socalforceblack}{%
  \socalkeepcolor{black}%
  \renewcommand{\color}[2][]{\socalkeepcolor{black}}%
  \renewcommand{\textcolor}[3][]{##3}%
}
\newcommand{\formalpanel}[2][\linewidth]{%
  \begingroup
  \socalforceblack
  \begin{minipage}[t]{#1}
    #2
  \end{minipage}%
  \endgroup
}

\newcommand{\formalcontentpanel}[3][\linewidth]{%
  \formalpanel[#1]{%
    \formalpaneltitle{#2}%
    \begingroup
    \formalcontentfont
    \formalcontentsymbols
    #3%
    \endgroup
  }%
}

\newcommand{\formalcontentblock}[2][\linewidth]{%
  \formalpanel[#1]{%
    \begingroup
    \formalcontentfont
    \formalcontentsymbols
    #2%
    \endgroup
  }%
}

\newcommand{\formalrulepanel}[3][\linewidth]{%
  \formalpanel[#1]{%
    \formalpaneltitle{#2}%
    \formalrulecontent{#3}%
  }%
}

\newcommand{\formalrulecontent}[1]{%
  \begingroup
  \formalrulefont
  \formalsymbols
  \setlength{\abovedisplayskip}{3pt}%
  \setlength{\belowdisplayskip}{3pt}%
  \setlength{\abovedisplayshortskip}{2pt}%
  \setlength{\belowdisplayshortskip}{2pt}%
  \begin{minipage}{\linewidth}
    \begin{mathpar}
      \mprset{flushleft}
      #1
    \end{mathpar}
  \end{minipage}
  \endgroup
}

\newcommand{\formalrulecolumn}[2][\linewidth]{%
  \begin{minipage}[t]{#1}
    \formalrulecontent{#2}%
  \end{minipage}%
}

\newcommand{\formalruleblock}[2][\linewidth]{%
  \formalpanel[#1]{%
    \formalrulecontent{#2}%
  }%
}


\newcommand{\socalflushdisplays}{%
  \renewcommand{\[}{\par\nobreak\vspace{1.0pt}\noindent$\displaystyle}%
  \renewcommand{\]}{$\par\vspace{1.0pt}}%
}
\newsavebox{\socalgrammarleft}
\newsavebox{\socalgrammarright}
\newlength{\socalgrammargap}
\newcommand{\socalgrammarcolumns}{%
  \sbox{\socalgrammarleft}{\begin{minipage}[t]{0.44\textwidth}
    \centering
    \input{formal_grammar_core}
  \end{minipage}}%
  \setlength{\socalgrammargap}{0pt}%
  \sbox{\socalgrammarright}{\begin{minipage}[t]{0.55\textwidth}
    \centering
    \input{formal_grammar_aux}
  \end{minipage}}%
  \setlength{\socalgrammargap}{\dimexpr\dp\socalgrammarleft-\dp\socalgrammarright\relax}%
  \ifdim\socalgrammargap<0pt \setlength{\socalgrammargap}{0pt}\fi
  \usebox{\socalgrammarleft}\hfill
  \begin{minipage}[t]{0.55\textwidth}
    \centering
    \input{formal_grammar_aux}
  \end{minipage}%
  \setlength{\socalgrammargap}{0pt}%
}
\newcommand{\socalgrammardisplays}{%
  \renewcommand{\[}{\par\nobreak\nointerlineskip\noindent$\displaystyle}%
  \renewcommand{\]}{$\par}%
}

\newsavebox{\socalrowL}
\newsavebox{\socalrowR}
\newlength{\socalrowdp}
\newcommand{\socalrulerow}[4]{%
  \par\vspace{1.0pt}%
  \noindent
  \sbox{\socalrowL}{\begin{minipage}[t]{#1\linewidth}#2\end{minipage}}%
  \sbox{\socalrowR}{\begin{minipage}[t]{#3\linewidth}#4\end{minipage}}%
  \setlength{\socalrowdp}{\dp\socalrowL}%
  \ifdim\dp\socalrowR>\socalrowdp \setlength{\socalrowdp}{\dp\socalrowR}\fi
  \usebox{\socalrowL}\hfill
  {\socalkeepcolor{FormalBorder}\vtop to \socalrowdp{%
    \cleaders\vbox to 2.2pt{\vss\hbox{\rule{0.7pt}{0.7pt}}\vss}\vfill}}%
  \hfill\usebox{\socalrowR}%
  \par\vspace{1.0pt}%
}

\newsavebox{\socalcolA}
\newsavebox{\socalcolB}
\newlength{\socalcolht}
\newcommand{\socalcolumnbox}[1]{\hsize=0.485\linewidth \linewidth=\hsize
  \parindent=0pt \parskip=0pt #1}
\newcommand{\socalrulecolumns}[2]{%
  \par\noindent
  \setbox\socalcolA=\vbox{\socalcolumnbox{#1}}%
  \setbox\socalcolB=\vbox{\socalcolumnbox{#2}}%
  \setlength{\socalcolht}{\ht\socalcolA}%
  \ifdim\ht\socalcolB>\socalcolht \setlength{\socalcolht}{\ht\socalcolB}\fi
  \hbox to \linewidth{\vbadness=10000
    \vbox to \socalcolht{\socalcolumnbox{#1}}%
    \hfill
    \vbox to \socalcolht{\socalcolumnbox{#2}}}%
  \par
}
\newcommand{\socaldottedline}{%
  \noindent{\socalkeepcolor{FormalBorder}\leaders\hbox to 2.2pt{\hss\rule[0.15ex]{0.7pt}{0.7pt}\hss}\hskip\linewidth}}
\newlength{\socalpairht}
\newcommand{\socalpairsep}{%
  \qquad\vcenter{\hbox{\socalkeepcolor{FormalBorder}\vbox to \socalpairht{%
    \cleaders\vbox to 2.2pt{\vss\hbox{\rule{0.7pt}{0.7pt}}\vss}\vfill}}}\qquad}
\newcommand{\socalpairfit}[1]{%
  \setlength{\socalpairht}{0pt}%
  \setbox0=\vbox{\hsize=\linewidth #1}%
  \setlength{\socalpairht}{\dimexpr\ht0+\dp0-3pt\relax}%
  #1}
\newcommand{\socalrulesep}{\par\vspace{2pt plus 1fill}\socaldottedline\par\vspace{3pt}}
\newcommand{\socalgroupsep}{\par\vspace{6pt}}

\newcommand{\socaljudgment}[2]{%
  \par\noindent
  {\textsc{#1}}\hfill{$#2$}\par
  \vspace{-1.5pt}\noindent{\socalkeepcolor{FormalBorder}\rule{\linewidth}{0.4pt}}\par
  \vspace{2pt}%
}

\newcommand{\socalbindctx}{%
  \ngRuleCtx\ngBind{\ngAlCtx'}{\AENV'}{\NENV'}{\UENV'}}
\newcommand{\socalJTyping}{%
  \socalbindctx\ngJT{\Theta}{\ngTyCtx}{\ngAlCtx}{\EXPR : \ngLocatedTy}{\ngAlCtx'}}
\newcommand{\socalJPattern}{%
  \socalbindctx\ngJPT{\Theta}{\TYP''@\ngLoc_s}{\ngTyCtx}{\ngAlCtx}{\pat : \ngLocatedTy}{\ngAlCtx'}}
\newcommand{\socalJProgram}{%
  \socalbindctx\ngJProgT{\Theta}{\PROG : \ngLocatedTy}{\ngAlCtx'}}
\newcommand{\socalJFun}{\ngJFunT{\Theta}{\FD}}
\newcommand{\socalJStep}{%
  \ngStepCfg{\Theta}{\STOR}{\MENV}{\EXPR}{\Theta'}{\STOR'}{\MENV'}{\EXPR'}}

\newcommand{\socalflushpremises}[1]{{\mprset{flushleft}#1}}

\newif\ifsocalwhereseen
\newcommand{\socalwhereright}[1]{{%
  \socalwhereseenfalse
  \renewcommand{\ngRuleWhere}[2]{\global\socalwhereseentrue
    \vcenter{\hbox{$\displaystyle ##1$}}\hspace{1.25em}\vcenter{\hbox{$\ngWhere{##2}$}}}%
  \renewcommand{\ngRuleWhereList}[2]{\global\socalwhereseentrue
    \vcenter{\hbox{$\displaystyle ##1$}}\hspace{1.25em}\vcenter{\hbox{$\ngWhereList{##2}$}}}%
  #1%
  \ifsocalwhereseen\else
    \PackageError{macros}{\string\socalwhereright: the wrapped rule has no
      where-block form it knows (\string\ngRuleWhere, \string\ngRuleWhereList)}{The
      formalism changed how a rule writes its where-block. Teach
      \string\socalwhereright\space the new form (macros.tex).}%
  \fi}}
\newcommand{\socalcenterrules}{%
  \renewcommand{\[}{\par\nobreak\vspace{1.0pt}\noindent\hbox to\linewidth\bgroup\hfil$\displaystyle}%
  \renewcommand{\]}{$\hfil\egroup\par\vspace{1.0pt}}%
}

\newlength{\socalgcat}
\newlength{\socalgmv}
\newlength{\socalgdef}
\newcolumntype{G}{@{}w{l}{\socalgcat}@{\hspace{0.6em}}w{l}{\socalgmv}@{\hspace{0.45em}}w{c}{\socalgdef}@{\hspace{0.45em}}l@{}}
\newcolumntype{H}{@{}w{l}{\socalgmv}@{\hspace{0.45em}}w{c}{\socalgdef}@{\hspace{0.45em}}l@{}}
\newcommand{\socalgrammargrid}[2]{%
  \settowidth{\socalgcat}{#1}%
  \settowidth{\socalgmv}{$#2$}%
  \settowidth{\socalgdef}{$\gramdef$}}

\newcommand{\socalgrouplabel}[1]{\text{\scriptsize\itshape\socalkeepcolor{black!55}#1}}
\newcommand{\socalgrouprows}[1]{\begin{array}{@{}r@{\quad}l@{}}#1\end{array}}
\newcommand{\socalpremsep}{\qquad}
\newcommand{\socalgrammarhead}[1]{\par\noindent{\scriptsize\itshape\socalkeepcolor{black!55}#1}\par\nobreak}

\newcommand{\socalfraction}[2]{\hbox{\advance\hsize by -0.5em
  $\displaystyle{#1\vrule depth 0.8ex width 0pt\above 0.55pt \vrule height 2.4ex width 0pt #2}$}}
\newcommand{\socalrulerhythm}{%
  \mprset{vskip=0.55ex}%
  \mprset{myfraction=\socalfraction}%
  \renewcommand{\ngPremBlock}[1]{{\renewcommand{\arraystretch}{1.3}%
    \begin{array}{@{}l@{}}##1\end{array}}}%
  \renewcommand{\ngPremGap}{\\\noalign{\vskip 1.1ex}}%
  \renewcommand{\ngGroupGap}{\rule{0pt}{3.4ex}}%
}

\newcommand{\socalrulestack}[2][\linewidth]{%
  \formalpanel[#1]{%
    \begingroup
    \formalrulefont
    \formalsymbols
    \formalgrammarkeywords
    \socalflushdisplays
    \setlength{\parskip}{0pt}%
    \setlength{\parindent}{0pt}%
    \setlength{\jot}{0pt}%
    \setlength{\abovedisplayskip}{0pt}%
    \setlength{\belowdisplayskip}{0pt}%
    \setlength{\abovedisplayshortskip}{0pt}%
    \setlength{\belowdisplayshortskip}{0pt}%
    \mprset{sep=0.9em}%
    \socalrulerhythm
    #2%
    \endgroup
  }%
}


\definecolor{canaryblue}{HTML}{2916F5}
\definecolor{darkgreen}{HTML}{006400}
\definecolor{darkpink}{HTML}{CD00CD}
\definecolor{graygreen}{rgb}{0.3,0.5,0.3}
\definecolor{grayblue}{rgb}{0.2,0.2,0.6}
\definecolor{grayred}{rgb}{0.5,0.2,0.2}
\definecolor{crimsonred}{HTML}{990000}
\definecolor{irishgreen}{HTML}{08A04B}
\definecolor{darkviolet}{HTML}{9400D3}
\newcommand{\myblue}{NavyBlue}
\newcommand{\myred}{BrickRed}



\newcommand{\marmoset}{{\sc Marmoset}\xspace}

\newcommand{\ribbit}{{\sc Ribbit}\xspace}

\newcommand{\systemSolver}{{\sc M$_{\mathit{solver}}$}\xspace}
\newcommand{\systemGreedy}{{\sc M$_{\mathit{greedy}}$}\xspace}


\newcommand{\alignedPre}{{\sc Algn$_{\mathit{pre}}$}\xspace}
\newcommand{\alignedIn}{{\sc Algn$_{\mathit{in}}$}\xspace}
\newcommand{\alignedPost}{{\sc Algn$_{\mathit{post}}$}\xspace}


\newcommand{\misalignedPost}{{\sc Misalgn$_{\mathit{post}}$}\xspace}
\newcommand{\misalignedPre}{{\sc Misalgn$_{\mathit{pre}}$}\xspace}

\newcommand{\misalignedGen}{{\sc Misalgn}\xspace}
\newcommand{\alignedGen}{{\sc Algn}\xspace}



\newcommand{\systemlang}[0]{\ensuremath{\lambda_{M}}}

\newcommand{\gibbon}{\textsc{Gibbon}\xspace}

\newcommand{\relc}{{\sc RELC}\xspace}

\newcommand{\ghc}{{\sc Ghc}\xspace}

\newcommand{\mlton}{{\sc MLton}\xspace}

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}


\newcommand{\snum}[1]{{\num[round-precision=3,round-mode=figures,scientific-notation=true,output-exponent-marker = e]{#1}}}
\newcommand{\snumfour}[1]{{\num[round-precision=4,round-mode=figures,scientific-notation=true,output-exponent-marker = e]{#1}}}

\newcommand{\fnumthree}[1]{{\num[round-mode=places,round-precision=3, scientific-notation=false]{#1}}}
\newcommand{\fnumtwo}[1]{{\num[round-mode=places,round-precision=2, scientific-notation=false]{#1}}}

\def\cpp{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\footnotesize\bf ++}}}
\def\csharp{C\tikz[x=1em,y=\baselineskip]%
  \draw (0.125,0.15) -- ++(0.15,0.5)%
        (0.325,0.15) -- ++(0.15,0.5)%
        (0.05,0.3) -- ++(0.45,0.0)%
        (0.1,0.5) -- ++(0.45,0.0);}

\newcommand{\benchname}[1]{\textcolor{lipicsGray}{\sffamily\small\bfseries\mathversion{bold}#1}}


==> paper-formalism/formalism-macros/defs.tex <==



\DeclareRobustCommand{\oldcalc}[0]{\texorpdfstring{LoCal}{LoCal}\xspace}
\DeclareRobustCommand{\newcalc}[0]{\texorpdfstring{SoCal}{SoCal}\xspace}
\DeclareRobustCommand{\sysname}[0]{\newcalc}


\DeclareRobustCommand{\ourcalc}[0]{\sysname}

\DeclareRobustCommand{\colobus}[0]{\texorpdfstring{\textsc{Colobus}}{Colobus}\xspace}
\DeclareRobustCommand{\AoS}[0]{\texorpdfstring{\textsc{AoS}}{AoS}}
\DeclareRobustCommand{\SoA}[0]{\texorpdfstring{\textsc{SoA}}{SoA}}
\DeclareRobustCommand{\unfactored}[0]{flattened\xspace}
\DeclareRobustCommand{\hybridfactored}[0]{hybrid factored\xspace}
\DeclareRobustCommand{\fullyfactored}[0]{factored\xspace}
\newcommand{\soaidx}{\mathsf{soa}}
\newcommand{\locsoa}{\ensuremath{loc_{\soaidx}}}
\newcommand{\clocsoa}{\ensuremath{cloc_{\soaidx}}}
\newcommand{\regsoa}{\ensuremath{reg_{\soaidx}}}
\newcommand{\lamadt} [0]{HiCal\xspace}

\newcommand{\lamcur}[0]{NoCal\xspace}

\newcommand{\gramdef}{\; ::= \;}
\newcommand{\gramor}{\; | \;}
\newcommand{\keywd}[1]{\mathit{#1}}
\newcommand{\gramkw}[1]{\ifmmode\mathsf{#1}\else\textsf{#1}\fi}
\newcommand{\gramwd}[1]{\gramkw{#1}}
\newcommand{\sgramwd}[1]{\gramkw{#1}}
\newcommand{\skeywd}[1]{\mathit{#1}}

\newcommand{\PROG}{\keywd{top}}
\newcommand{\DD}{\keywd{dd}}
\newcommand{\VD}{\keywd{vd}}
\newcommand{\FD}{\keywd{fd}}
\newcommand{\DC}{\keywd{K}}
\newcommand{\sDC}{\skeywd{K}}
\newcommand{\TC}{\keywd{T}}
\newcommand{\EXPR}{\keywd{e}}
\newcommand{\sEXPR}{\skeywd{e}}
\newcommand{\DATA}{\gramwd{data}}
\newcommand{\Int}{\mathsf{Int}}             %
\newcommand{\TYP}{\keywd{\tau}}             %
\newcommand{\hTYP}{\keywd{\hat{\tau}}}      %
\newcommand{\sTYP}{\skeywd{\tau}}
\newcommand{\dTYP}{\keywd{\widetilde{\tau}}}    %
\newcommand{\var}{\svar}
\newcommand{\svar}{x}
\newcommand{\fvar}{\sfvar}
\newcommand{\sfvar}{f}
\newcommand{\yvar}{y}
\newcommand{\num}{n}
\newcommand{\ARROW}{\rightarrow}
\newcommand{\RP}{\keywd{dl}}
\newcommand{\sRP}{\skeywd{dl}}
\newcommand{\loc}{\skeywd{l}}
\newcommand{\locvec}{\vec{l}}
\newcommand{\storeaddr}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\concreteloc}[3]{\ensuremath{\langle #1, #2 \rangle ^{#3}}}

\newcommand{\concretelocvec}[3]{%
  \ensuremath{%
    \left\langle
      \vec{\mathord{\scriptstyle #1}},\,
      \vec{\mathord{\scriptstyle #2}}
    \right\rangle^{%
      \smash{\vec{\mathord{\scriptscriptstyle #3}}}%
    }%
  }%
}


\newcommand{\reg}{\skeywd{r}}
\newcommand{\regvec}{\vec{r}}
\newcommand{\sreg}{\skeywd{r}}
\newcommand{\LS}{\keywd{ls}}
\newcommand{\LC}{\keywd{lc}}
\newcommand{\LE}{\keywd{le}}
\newcommand{\FLDS}{\keywd{flds}}
\newcommand{\letpack}[3]{\gramwd{let}\;#1=#2\;\gramwd{in}\;#3}
\newcommand{\letloc}[3]{\gramwd{letloc}\;#1 = #2\;\gramwd{in}\;#3}
\newcommand{\letlocvec}[3]{\gramwd{letloc_{vec}}\;#1 = #2\;\gramwd{in}\;#3}
\newcommand{\letreg}[2]{\gramwd{letregion}\;#1\;\gramwd{in}\;#2}
\newcommand{\fapp}[2]{\fvar \;[#1]\; #2}
\newcommand{\TS}{\keywd{ts}}
\newcommand{\ssetbool}[4]{#4 = #3[#2\mapsto \keywd{#1}=\keywd{True}]}
\newcommand{\sinlinesetbool}[3]{#3[#2\mapsto \keywd{#1}=\keywd{True}]}
\newcommand{\CS}{\keywd{cs}}
\newcommand{\pat}{\keywd{pat}}
\newcommand{\ptr}[2]{(\gramwd{ptr}\;\keywd{#1}\;\keywd{#2})}
\newcommand{\sind}{i}
\newcommand{\ind}{\keywd{i}}
\newcommand{\indj}{\keywd{j}}
\newcommand{\intn}{\keywd{n}}

\newcommand{\indvec}{\vec{\keywd{i}}}
\newcommand{\indjvec}{\vec{\keywd{j}}}

\newcommand{\VAL}{\keywd{v}}
\newcommand{\sVAL}{\keywd{sv}}
\newcommand{\ec}{\keywd{\mathcal{E}}}
\newcommand{\evalc}[1]{\ec \llbracket #1 \rrbracket }
\newcommand{\STOR}{\keywd{S}}
\newcommand{\stepsto}{\;\hookrightarrow\;}
\newcommand{\Name}{\Red{Name }}
\newcommand{\q}[1]{\texttt{#1}}
\newcommand{\frl}[1]{{\ensuremath \mathit{frl}(#1)}}
\newcommand{\caseclause}[2]{#1 \;\rightarrow \;#2}
\newcommand{\case}[2]{\gramwd{case}\; #1 \;\gramwd{of}\;#2}
\newcommand{\spat}{\keywd{spat}}
\newcommand{\switch}[2]{\gramwd{switch}\; #1 \;\gramwd{of}\;#2}
\newcommand{\readInt}[1]{\gramwd{readInt} \; #1}
\newcommand{\writeInt}[2]{\gramwd{writeInt} \; #1 \; #2}
\newcommand{\readTag}[1]{\gramwd{readTag} \; #1}
\newcommand{\writeTag}[2]{\gramwd{writeTag} \; #1 \; #2}
\newcommand{\readCursor}[1]{\gramwd{readCursor} \; #1}
\newcommand{\writeCursor}[2]{\gramwd{writeCursor} \; #1 \; #2}
\newcommand{\addCursor}[2]{\gramwd{addCursor} \; #1 \; #2}
\newcommand{\makeCursorArray}[2]{\gramwd{makeCursorArray} \; #1 \; [#2]}
\newcommand{\indexCursorArray}[2]{\gramwd{indexCursorArray} \; #1 \; #2}
\newcommand{\writeCursorMutable}[2]{\gramwd{writeCursorMutable} \; #1 \; #2}
\newcommand{\addrOfCursor}[1]{\gramwd{addrOfCursor} \; #1}
\newcommand{\derefMutCursor}[1]{\gramwd{derefMutCursor} \; #1}
\newcommand{\bumpMutableCursor}[2]{\gramwd{bumpMutCursor} \; #1 \; #2}
\newcommand{\datacon}[3]{\ensuremath{#1 \;#2 \;#3}}
\newcommand{\litcon}[2]{\datacon{\keywd{L}}{#1}{#2}}
\newcommand{\litnum}{\keywd{n}}
\newcommand{\CP}{\keywd{cp}}
\newcommand{\tptr}[3]{\langle \mathit{ptr}\;#2\;#3 \rangle_{#1}}
\newcommand{\LM}{\keywd{M}}
\newcommand{\locis}[2]{\ensuremath{#1:#2}}
\newcommand{\lvar}{\keywd{lx}}
\newcommand{\has}[3]{\ensuremath{#1(#2) = #3}}
\newcommand{\zeroidx}[1]{\ensuremath{\mathsf{ZeroIdx}(#1)}}
\newcommand{\startr}[1]{(\gramwd{start}\; #1)}
\newcommand{\startrvec}[1]{(\gramwd{start_{vec}}\; #1)}
\newcommand{\afterl}[1]{(\gramwd{after}\; #1)}
\newcommand{\afterlvec}[1]{(\gramwd{after_{vec}}\; #1)}
\newcommand{\getDconLoc}[1]{(\gramwd{projTagLoc}\; #1)}
\newcommand{\getFieldLoc}[2]{(\gramwd{projFieldLoc}\;#1\;#2)}
\newcommand{\getFieldLocVector}[2]{(\gramwd{projFieldLoc_{vec}}\;#1\;#2)}
\newcommand{\getDconLocAbbr}{\mathit{gdc}}
\newcommand{\getFieldLocAbbr}{\mathit{gfl}}
\newcommand{\mkSoALocAbbr}{\mathit{msl}}
\newcommand{\makevectorloc}[2]{(\gramwd{introLocVec}\;#1\;#2)}
\newcommand{\makevectorregion}[2]{(\gramwd{mkSoAReg}\;#1\;#2)}
\newcommand{\soaentry}[3]{(\mathsf{#1}, #2, #3)}
\newcommand{\soaalist}[3]{\overharpoon{\soaentry{#1}{#2}{#3}}}
\newcommand{\soaloc}[5]{\locreg{#1}{#2}\,\soaentry{#3}{#4}{#5}}
\newcommand{\soacloc}[6]{\concreteloc{#1}{#2}{#3}\,\soaentry{#4}{#5}{#6}}
\newcommand{\soareg}[4]{#1\,\soaentry{#2}{#3}{#4}}
\newcommand{\soaloclist}[5]{\locreg{#1}{#2}\,\soaalist{#3}{#4}{#5}}
\newcommand{\soacloclist}[6]{\concreteloc{#1}{#2}{#3}\,\soaalist{#4}{#5}{#6}}
\newcommand{\soareglist}[4]{#1\,\soaalist{#2}{#3}{#4}}
\newcommand{\tightoverset}[2]{%
  \mathop{#2}\limits^{\vbox to -.5ex{\kern-0.75ex\hbox{$#1$}\vss}}}
\newcommand\set[1]{\{ \, \ensuremath{#1} \,\}}
\newcommand{\ecdot}{\bullet}
\newcommand{\heap}{\keywd{h}}
\newcommand{\alphaequiv}{=_{\alpha}}

\newcommand{\LENV}{\keywd{L}}
\newcommand{\RENV}{\keywd{R}}
\newcommand{\CENV}{\keywd{C}}
\newcommand{\TENV}{\keywd{\Gamma}}
\newcommand{\EENV}{\keywd{E}}
\newcommand{\SENV}{\keywd{\Sigma}}
\newcommand{\MENV}{\keywd{M}}
\newcommand{\FENV}{\keywd{F}}
\newcommand{\AENV}{\keywd{A}}
\newcommand{\NENV}{\keywd{N}}

\newcommand{\inloc}[0]{\ensuremath{\downarrow\sloc}}
\newcommand{\outloc}[0]{\ensuremath{\uparrow\sloc}}
\newcommand{\locreg}[2]{\ensuremath{{#1}^{#2}}}
\newcommand{\locregstd}{\ensuremath{{\loc}^{\reg}}}
\newcommand{\locregvec}[2]{\ensuremath{\vec{#1}^{\,\vec{#2}}}}



\newcommand{\tyatlocreg}[3]{#1 \ensuremath{@} \locreg{#2}{#3}}
\newcommand{\tyatlocregvec}[3]{#1 \ensuremath{@} \locregvec{#2}{#3}}

\newcommand{\tyatlocregvecnewloc}[2]{#1 \ensuremath{@} loc_{#2}}

\newcommand{\tyatlocregvecnewlocdiff}[3]{#1 \ensuremath{@} loc_{#2}^{#3}}

\newcommand{\Cursorize}[0]{Cursorize}
\newcommand{\fresh}[0]{\keywd{fresh}}

\newcommand{\Single}[1]{\keywd{Single}\;#1}
\newcommand{\Vector}[1]{\keywd{Vector}\;#1}


\newcommand{\subst}[3]{\ensuremath{#1[#3/#2]}}

\newcommand{\typeofcon}{\keywd{TypeOfCon}}
\newcommand{\typeoffield}{\keywd{TypeOfField}}
\newcommand{\kargtys}{\keywd{ArgTysOfConstructor}}
\newcommand{\allocptr}[2]{\keywd{MaxIdx}(#1,#2)}
\newcommand{\valididx}[1]{\ensuremath{\mathsf{ValidIdx}(#1)}}

\newcommand{\ctors}[1]{\keywd{Ctors}(#1)}
\newcommand{\fields}[1]{\keywd{Fields}(#1)}
\newcommand{\liftmap}[1]{\mu(#1)}
\newcommand{\zeromap}[1]{\MENV_Z(#1)}



\newcommand{\Iscalar}{\keywd{I}_{\mathsf{scal}}}

\newcommand{\update}[3]{\ensuremath{#1+\{#2 \mapsto #3\}}}

\newcommand{\ewitnessentails}{\ensuremath{\vdash_{\mathit{ew}}}}
\newcommand{\ewitness}[4]{\ensuremath{#1;#2;#3 \ewitnessentails\, #4}}
\newcommand{\ewitnessrecentails}{\ensuremath{\vdash_{\mathit{ew}_\mathit{rec}}}}
\newcommand{\ewitnessrec}[4]{\ensuremath{#1;#2;#3 \ewitnessrecentails #4}}
\newcommand{\storewfentails}{\ensuremath{\vdash_{\mathit{wf}}}}
\newcommand{\storewf}[6]{\ensuremath{#1;#2;#3;#4 \storewfentails #5;#6}}
\newcommand{\storewfcfa}[3]{\ensuremath{#1 \vdash_{wf_{cfc}} #2;#3}}
\newcommand{\storewfca}[4]{\ensuremath{#1;#2 \vdash_{wf_{ca}} #3;#4}}

\newcommand{\tcfun}{\ensuremath{\vdash_{fun}}}
\newcommand{\tcpat}{\ensuremath{\vdash_{pat}}}
\newcommand{\tcts}{\ensuremath{\vdash_{ts}}}

\newcommand{\refwellformed}[2]{WF~\ref{#1};\ref{#2}}
\newcommand{\refendwitness}[2]{EW~\ref{#1};\ref{#2}}
\newcommand{\refts}[1]{T-#1}
\newcommand{\refcase}[1]{Case-\ref{#1}}
\newcommand{\elimexists}[0]{$\exists$ elim}
\newcommand{\refinst}[0]{Inst.}

\newcommand{\tfunctiondef}{T-Function-Definition}
\newcommand{\tdatacon}{T-DataConstructor}
\newcommand{\tdataconfullyfactored}{T-DataConstructor-FullyFactored}
\newcommand{\tdataconfullyfactoredanyordering}{T-DataConstructor-FullyFactored-Any-Ordering}
\newcommand{\ddatacon}{D-DataConstructor}       %
\newcommand{\ddataconfullyfactored}{D-DataConstructor-FullyFactored}
\newcommand{\dletloctag}{D-LetLoc-Tag}
\newcommand{\dletlocafter}{D-LetLoc-After}
\newcommand{\dletlocstart}{D-LetLoc-Start}
\newcommand{\dletlocprojtag}{D-LetLoc-ProjTag}
\newcommand{\dletlocprojfield}{D-LetLoc-ProjField}
\newcommand{\dletlocintrovec}{D-LetLoc-IntroLocVec}
\newcommand{\dapp}{D-App}
\newcommand{\dletregion}{D-LetRegion}
\newcommand{\tcase}{T-Case}
\newcommand{\dcase}{D-Case}
\newcommand{\dcasefullyfactored}{D-Case}%
\newcommand{\valididxfullyfactored}{ValidIdx-FullyFactored}
\newcommand{\ddataconsoa}{\ddataconfullyfactored}
\newcommand{\dcasesoa}{\dcasefullyfactored}
\newcommand{\tpat}{T-Pattern}
\newcommand{\tprogram}{T-Program}
\newcommand{\tllafter}{T-LetLoc-After}
\newcommand{\tlltag}{T-LetLoc-Tag}
\newcommand{\tlltagvector}{T-LetLoc-ProjTag}
\newcommand{\tllfieldvector}{T-LetLoc-ProjField}
\newcommand{\tllmakeSoA}{T-LetLoc-IntroLocVec}
\newcommand{\tllstart}{T-LetLoc-Start}
\newcommand{\tlregion}{T-LetRegion}
\newcommand{\tvar}{T-Var}
\newcommand{\tlet}{T-Let}
\newcommand{\dletexp}{D-Let-Expr}
\newcommand{\dletval}{D-Let-Val}
\newcommand{\tapp}{T-App}
\newcommand{\tconcreteloc}{T-Concrete-Loc}
\newcommand{\tint}{T-Int}

\newcommand{\emptytenv}{\emptyset}



\newcommand\mydots{\ifmmode{...}\else\makebox[1em][c]{.\hfil.\hfil.}\fi}


==> paper-formalism/formalism-macros/socal-macros.tex <==

\newcommand{\ngLoc}{\keywd{L}}          %
\newcommand{\ngReg}{\keywd{R}}          %
\newcommand{\packs}{\mathrel{\vartriangleright}}
\newcommand{\letregty}[3]{\gramkw{letregion}\;#1 : #2\;\gramkw{in}\;#3}
\newcommand{\ngZeroCursor}[1]{\mathrm{zeroCursor}(#1)}
\newcommand{\ngAdvTags}[2]{\gramkw{advanceTags}\;#1\;\gramkw{for}\;#2}
\newcommand{\ngAdvField}[4]{\gramkw{advanceField}\;#1\;(#2,#3)\;%
  \gramkw{beyond}\;#4}
\newcommand{\ngPath}{\keywd{\pi}}
\newcommand{\ngEmptyPath}{\keywd{\epsilon}}
\newcommand{\ngPos}{\keywd{\rho}}
\newcommand{\ngFieldKey}[2]{(#1,#2)}
\newcommand{\ngPathsOf}[1]{\mathrm{paths}(#1)}
\newcommand{\ngBaseReg}{\keywd{r}}      %

\newcommand{\ngCurs}[1]{\ensuremath{\langle #1\rangle}}
\newcommand{\ngCell}[2]{\ensuremath{#1[#2]}}
\newcommand{\ngLayoutCursorT}[1]{\ensuremath{\mathrm{LayoutCursor}(#1)}}
\newcommand{\ngFactored}[1]{\ensuremath{\mathrm{Fac}(#1)}}
\newcommand{\ngProj}[2]{\ensuremath{#1\!\downarrow\!#2}}
\newcommand{\ngTagNext}[1]{\ensuremath{\mathrm{tagNext}(#1)}}
\newcommand{\ngReplace}[3]{\ensuremath{#1[#2 := #3]}}
\newcommand{\ngFitsO}[2]{\ensuremath{#1 \mathrel{\mathrm{fits}^{\mathcal{O}}} #2}}
\newcommand{\ngEraseC}[1]{\ensuremath{\lfloor #1 \rfloor_{\mathrm{c}}}}
\newcommand{\ngReifyC}[1]{\ensuremath{\lceil #1 \rceil_{\mathrm{c}}}}
\newcommand{\ngLocatedTy}{\keywd{\hat\tau}}
\newcommand{\ngFreshFor}[2]{#1 \mathrel{\#} #2}
\newcommand{\ngFresh}[2]{\mathrm{fresh}(#1;\,#2)}
\newcommand{\ngTypeScheme}{\keywd{ts}}
\newcommand{\ngLE}{\keywd{le}}
\newcommand{\ngAP}{\keywd{ap}}
\newcommand{\ngAtom}{\ensuremath{\mathrm{Atom}}}
\newcommand{\ngEraseA}[1]{\ensuremath{\mathrm{erase}_A(#1)}}
\newcommand{\ngAFam}[1]{\ensuremath{\mathrm{AFamily}(#1)}}
\newcommand{\ngUnstarted}{\ensuremath{\gramkw{unstarted}}}
\newcommand{\ngStarted}[1]{\ensuremath{\gramkw{started}(#1)}}
\newcommand{\ngEntry}[2]{\ensuremath{\mathrm{entry}(#1,#2)}}
\newcommand{\ngRegionsOf}[1]{\ensuremath{\mathrm{regions}(#1)}}
\newcommand{\ngPositionsOf}[1]{\ensuremath{\mathrm{positions}(#1)}}
\newcommand{\ngFam}{\ensuremath{F}}
\newcommand{\ngConstFam}[1]{\ensuremath{F_{#1}}}
\newcommand{\ngDesc}[2]{\ensuremath{\mathrm{desc}_{#1}(#2)}}
\newcommand{\ngDescOverride}[4]{\ensuremath{#1[\ngDesc{#2}{#3} \mapsto #4]}}

\newcommand{\ngLocatedTySub}[1]{\keywd{\hat\tau_{#1}}}
\newcommand{\ngAfterTy}[1]{(\gramkw{after}\;#1)}
\newcommand{\ngStartRegTy}[2]{(\gramkw{start}\;#1\!:\!#2)}
\newcommand{\ngDom}[1]{\mathrm{dom}(#1)}
\newcommand{\vwf}[5]{#1 \vdash^{#2}_{\mathit{val}} #3 : #4 \rightsquigarrow #5}
\newcommand{\ngTypeAt}[2]{\mathrm{typeAt}(#1,#2)}
\newcommand{\crealj}[3]{#1 \vdash_{\mathit{cr}} #2 \,;\, #3}
\newcommand{\allocwfj}[4]{#1;#2 \vdash_{\mathit{alloc}} #3 \,;\, #4}
\newcommand{\storewfj}[7]{#1;#2;#3;#4;#5 \vdash_{\mathit{wf}} #6;#7}
\newcommand{\storewfjO}[8]{#1;#2;#3;#4;#5
  \vdash_{\mathit{wf}}^{\mathcal{O}} #6;#7;#8}
\newcommand{\ngRedArrow}{\longrightarrow}
\newcommand{\ngStepsto}{\;\ngRedArrow\;}
\newcommand{\ngStepW}[4]{#1 \vdash #2 \ngStepsto #3 \dashv #4}
\newcommand{\ngStepWB}[4]{#1 \vdash #2 \ngStepstoB #3 \dashv #4}
\newcommand{\ngStepWStar}[4]{#1 \vdash #2 \ngStepstoStar #3 \dashv #4}
\newcommand{\ngCfg}[4]{\ngThetaCheck{#1}\langle #1;\, #2;\, #3;\, #4\rangle}
\newcommand{\ngStepCfg}[8]{%
  \ngCfg{#1}{#2}{#3}{#4} \ngStepsto \ngCfg{#5}{#6}{#7}{#8}}
\newcommand{\ngStepCfgB}[8]{%
  \ngCfg{#1}{#2}{#3}{#4} \ngStepstoB \ngCfg{#5}{#6}{#7}{#8}}
\newcommand{\ngStepCfgStar}[8]{%
  \ngCfg{#1}{#2}{#3}{#4} \;\ngRedArrow^*\; \ngCfg{#5}{#6}{#7}{#8}}
\newcommand{\ngStepCfgLong}[8]{%
  \begin{array}[b]{@{}l@{}}\ngCfg{#1}{#2}{#3}{#4} \\
    \quad {\ngStepsto} \ngCfg{#5}{#6}{#7}{#8}\end{array}}
\newcommand{\ngStepCfgBLong}[8]{%
  \begin{array}[b]{@{}l@{}}\ngCfg{#1}{#2}{#3}{#4} \\
    \quad {\ngStepstoB}\; \ngCfg{#5}{#6}{#7}{#8}\end{array}}
\newcommand{\ngStepCfgStarLong}[8]{%
  \begin{array}[b]{@{}l@{}}\ngCfg{#1}{#2}{#3}{#4} \\
    \quad {\;\ngRedArrow^*\;} \ngCfg{#5}{#6}{#7}{#8}\end{array}}
\newcommand{\Coherent}[2]{\mathrm{Coherent}(#1,#2)}
\newcommand{\ngMaxIdx}[2]{\ensuremath{\mathrm{MaxIdx}(#1,#2)}}
\newcommand{\ngFront}[1]{\ensuremath{\mathrm{front}(#1)}}
\newcommand{\ngMemFront}[1]{\ensuremath{\mathrm{mfront}(#1)}}
\newcommand{\ngFootprint}[1]{\ensuremath{\mathrm{reads}(#1)}}
\newcommand{\ngAllocatedPositions}[1]{\ensuremath{\mathrm{AllocatedPositions}(#1)}}
\newcommand{\ngBackOf}[1]{\ensuremath{\mathrm{back}(#1)}}
\newcommand{\ngTrim}[2]{\ensuremath{\mathrm{trim}(#1,#2)}}
\newcommand{\UENV}{\keywd{U}}

\newcommand{\wfdecl}{\ensuremath{\vdash_{\mathit{data}}}}

\newcommand{\ngFieldChain}[5]{#1 \vdash #2 \mathrel{\rightarrowtail_{#3,#4}} #5}
\newcommand{\ngFieldLinks}[1]{\mathrm{fieldLinks}(#1)}
\newcommand{\ngSources}[1]{\mathrm{sources}(#1)}
\newcommand{\ngEndOf}[1]{\mathrm{end}(#1)}
\newcommand{\ngChainRoot}[2]{\mathrm{root}_{#1}(#2)}

\newcommand{\ngLocVal}[1]{\ensuremath{\mathrm{locval}(#1)}}
\newcommand{\ngAtLocO}[2]{#1\mathord{@}^{\mathcal{O}}#2}

\newcommand{\ngCtx}{\mathcal{E}}
\newcommand{\ngCtxFill}[2]{#1[#2]}
\newcommand{\ngNadd}{\Delta\NENV}
\newcommand{\ngStepstoB}{\Longrightarrow_{b}}
\newcommand{\ngCells}[1]{\|#1\|}
\newcommand{\ngPSetO}{\ensuremath{\mathbb{P}^{\mathcal{O}}}}
\newcommand{\ngEraseP}[1]{\lfloor #1 \rfloor_{\mathrm{p}}}
\newcommand{\ngReifyP}[1]{\lceil #1 \rceil_{\mathrm{p}}}
\newcommand{\ngLog}{\ensuremath{\mathcal{L}}}          %
\newcommand{\ngWLog}[1]{\ensuremath{\mathrm{WriteLog}(#1)}}
\newcommand{\ngSnoc}[3]{\ensuremath{#1 \cdot (#2,#3)}} %
\newcommand{\ngLen}[1]{\ensuremath{|#1|}}              %
\newcommand{\ngAddrs}[1]{\ensuremath{\mathrm{addrs}(#1)}}
\newcommand{\ngStampOf}[2]{\ensuremath{\mathrm{stamp}_{#1}(#2)}}
\newcommand{\ngEraseW}[1]{\lfloor #1 \rfloor_{\mathrm{w}}}
\newcommand{\ngReifyW}[1]{\lceil #1 \rceil_{\mathrm{w}}}
\newcommand{\ngErase}[1]{\lfloor #1 \rfloor}
\newcommand{\ngErasePos}[1]{\lfloor #1 \rfloor_{\mathrm{pos}}}
\newcommand{\ngEraseS}[1]{\lfloor #1 \rfloor_{\SENV}}
\newcommand{\ngReifyS}[1]{\lceil #1 \rceil_{\SENV}}
\newcommand{\ngEraseV}[2]{\lfloor #2 \rfloor^{#1}_{\mathrm{v}}}
\newcommand{\ngReifyV}[2]{\lceil #2 \rceil^{#1}_{\mathrm{v}}}

\newcommand{\ngOpenCell}[1]{%
  \tikz[baseline=(c.base)]{\node[shape=circle,draw,very thick,
    inner sep=0.5pt] (c) {#1};}%
}

\newcommand{\ngTyCtx}{\keywd{\Psi}}
\newcommand{\ngAlCtx}{\keywd{\Omega}}
\newcommand{\ngBind}[4]{%
  \expandafter\def\csname ngBind:\detokenize{#1}\endcsname##1{#2##1#3##1#4}}
\newcommand{\ngLookup}[2]{%
  \ifcsname ngBind:\detokenize{#1}\endcsname
    \csname ngBind:\detokenize{#1}\endcsname{#2}%
  \else
    \PackageError{socal-macros}{No tuple declared for \detokenize{#1}}%
      {Declare the tuple in the enclosing group.}%
  \fi}
\newcommand{\ngShow}[1]{#1 = (\ngLookup{#1}{,\,})}
\newcommand{\ngShowAt}[1]{#1 &= (\ngLookup{#1}{,\,})}
\newcommand{\ngTup}[3]{\ifdefined\ngExpandJudgmentsBuild #1;#2;#3\else(#1,\,#2,\,#3)\fi}
\newcommand{\ngArg}[1]{\ngArgSplit#1\ngArgEnd{#1}}
\newcommand{\ngArgSplit}{}
\def\ngArgSplit#1#2\ngArgEnd#3{%
  \expandafter\ifx\csname ngTup\endcsname#1#3\else\ngLookup{#3}{;}\fi}
\newcommand{\ngArgCheck}[1]{\setbox0\hbox{$\ngArg{#1}$}}
\newcommand{\ngThetaBad}{%
  \PackageError{socal-macros}{A region typing environment argument is a
    grouped context}{The first argument of a judgment with Theta is the
    region typing environment, not a context.}}
\newcommand{\ngThetaFirst}{}
\def\ngThetaFirst#1#2\ngArgEnd{%
  \ifx\ngTyCtx#1\ngThetaBad\fi
  \ifx\ngAlCtx#1\ngThetaBad\fi
  \expandafter\ifx\csname ngTup\endcsname#1\ngThetaBad\fi}
\newcommand{\ngThetaCheck}[1]{%
  \if\relax\detokenize{#1}\relax
    \PackageError{socal-macros}{Empty region typing environment argument}%
      {Write the region typing environment the judgment is read at.}%
  \else\setbox0\hbox{$\ngThetaFirst#1\ngArgEnd$}\fi}
\newcommand{\ngJ}[4]{\ifdefined\ngExpandJudgmentsBuild
    \ngArg{#1};\ngArg{#2} \vdash \ngArg{#4};\, #3%
  \else
    \ngArgCheck{#1}\ngArgCheck{#2}\ngArgCheck{#4}%
    #1;\,#2 \vdash #3 \dashv #4%
  \fi}
\newcommand{\ngJT}[5]{\ngThetaCheck{#1}\ifdefined\ngExpandJudgmentsBuild
    #1;\; \ngArg{#2};\ngArg{#3} \vdash \ngArg{#5};\, #4%
  \else
    \ngArgCheck{#2}\ngArgCheck{#3}\ngArgCheck{#5}%
    #1;\;#2;\,#3 \vdash #4 \dashv #5%
  \fi}
\newcommand{\ngJPT}[6]{\ngThetaCheck{#1}\ifdefined\ngExpandJudgmentsBuild
    #1;\; #2;\ngArg{#3};\ngArg{#4} \tcpat \ngArg{#6};\, #5%
  \else
    \ngArgCheck{#3}\ngArgCheck{#4}\ngArgCheck{#6}%
    #1;\;#2;\,#3;\,#4 \tcpat #5 \dashv #6%
  \fi}
\newcommand{\ngJFunT}[2]{\ngThetaCheck{#1}#1 \tcfun #2}
\newcommand{\ngJProgT}[3]{\ngThetaCheck{#1}\ifdefined\ngExpandJudgmentsBuild
    #1 \vdash_{\mathit{prog}}\; \ngArg{#3};\; #2%
  \else
    \ngArgCheck{#3}%
    #1 \vdash_{\mathit{prog}} #2 \dashv #3%
  \fi}
\newcommand{\ngJP}[5]{\ifdefined\ngExpandJudgmentsBuild
    #1;\ngArg{#2};\ngArg{#3} \tcpat \ngArg{#5};\, #4%
  \else
    \ngArgCheck{#2}\ngArgCheck{#3}\ngArgCheck{#5}%
    #1;\,#2;\,#3 \tcpat #4 \dashv #5%
  \fi}
\newcommand{\ngJProg}[2]{\ifdefined\ngExpandJudgmentsBuild
    \vdash_{\mathit{prog}}\; \ngArg{#2};\; #1%
  \else
    \ngArgCheck{#2}%
    \vdash_{\mathit{prog}}\; #1 \dashv #2%
  \fi}
\newcommand{\ngJHead}[2]{\ifdefined\ngExpandJudgmentsBuild
    \ngArg{#1};\ngArg{#2}%
  \else
    \ngArgCheck{#1}\ngArgCheck{#2}#1;\,#2%
  \fi}
\newcommand{\ngJTail}[2]{\ifdefined\ngExpandJudgmentsBuild
    \vdash \ngArg{#2};\, #1%
  \else
    \ngArgCheck{#2}\vdash #1 \dashv #2%
  \fi}
\newcommand{\ngJLong}[4]{%
  \begin{array}[b]{@{}l@{}}\ngJHead{#1}{#2} \\ \quad \ngJTail{#3}{#4}\end{array}}
\newcommand{\ngJHeadT}[3]{\ngThetaCheck{#1}\ifdefined\ngExpandJudgmentsBuild
    #1;\; \ngArg{#2};\ngArg{#3}%
  \else
    \ngArgCheck{#2}\ngArgCheck{#3}#1;\;#2;\,#3%
  \fi}
\newcommand{\ngJLongT}[5]{%
  \begin{array}[b]{@{}l@{}}\ngJHeadT{#1}{#2}{#3} \\ \quad \ngJTail{#4}{#5}\end{array}}
\newcommand{\ngTupList}[3]{#1,#2,#3}
\newcommand{\ngArgList}[1]{\ngArgListSplit#1\ngArgEnd{#1}}
\newcommand{\ngArgListSplit}{}
\def\ngArgListSplit#1#2\ngArgEnd#3{%
  \expandafter\ifx\csname ngTup\endcsname#1{\expandafter\let\csname ngTup\endcsname\ngTupList#3}%
  \else\ngLookup{#3}{,}\fi}
\newcommand{\ngFreshCtx}[3]{\ifdefined\ngExpandJudgmentsBuild
    \ngFresh{#1}{\ngArgList{#2},\ngArgList{#3}}%
  \else
    \ngArgCheck{#2}\ngArgCheck{#3}%
    \ngFresh{#1}{#2,#3}%
  \fi}
\newcommand{\ngRuleCtx}{%
  \ngBind{\ngTyCtx}{\TENV}{\SENV}{\CENV}%
  \ngBind{\ngAlCtx}{\AENV}{\NENV}{\UENV}}
\newcommand{\ngAnn}{\TYP_{\mathrm{ann}}}
\newcommand{\ngPremBlock}[1]{{\begin{array}{@{}l@{}}#1\end{array}}}
\newcommand{\ngPremGap}{\\\noalign{\vskip 1.2ex}}
\newcommand{\ngQuantBody}[2]{#1\begin{array}[t]{@{}l@{}}#2\end{array}}
\newcommand{\ngVecClear}{\rule{0pt}{3.2ex}}
\newcommand{\ngGroupGap}{\rule{0pt}{3.4ex}}
\newcommand{\ngWhere}[1]{\text{where}\;\;\begin{aligned}[t]#1\end{aligned}}
\newcommand{\ngRuleWhere}[2]{%
  \begin{array}{@{}l@{}}#1\\[1.2ex]\quad\ngWhere{#2}\end{array}}
\newcommand{\ngWhereList}[1]{\text{where}\;\;%
  {\renewcommand{\arraystretch}{1.25}\begin{array}[t]{@{}l@{}}#1\end{array}}}
\newcommand{\ngWhereCont}{\quad}
\newcommand{\ngRuleWhereList}[2]{%
  \begin{array}{@{}l@{}}#1\\[1.2ex]\quad\ngWhereList{#2}\end{array}}


==> paper-formalism/paper-fragments/gr-datadecl.tex <==
\[
  \begin{array}{G}
    \textup{Datatype Declarations} & \DD & \gramdef &
      \DATA\;\dTYP = \overharpoon{\DC\;\overharpoon{\TYP}} \\
    \textup{Types} & \TYP & \gramdef & \dTYP
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-env-core.tex <==
\[
  \begin{array}{H}
    \Theta & \gramdef & \set{\ngReg_1 \mapsto \TYP_1, \ldots} \\
    \TENV & \gramdef & \set{\var_1 \mapsto \ngLocatedTy_1, \ldots} \\
    \SENV,\NENV,\UENV & \gramdef & \set{\ngLoc_1^{\ngPos_1}, \ldots} \\
    \CENV & \gramdef & \set{\ngLoc_1^{\ngPos_1} \mapsto \ngLE_1, \ldots}
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-env-regiontyped.tex <==
\[
  \begin{array}{H}
  \AENV & \gramdef & \set{\ngReg_1 \mapsto \ngAP_1, \ldots}
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-functiondecl.tex <==
\[
  \begin{array}{G}
  \textup{Function Declarations} & \FD & \gramdef &
      \fvar : \ngTypeScheme \;;\; \fvar\,\overharpoon{\var} = \EXPR
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-locatedtypes-scheme.tex <==
\[
  \begin{array}{G}
  \textup{Located Types} & \ngLocatedTy & \gramdef &
  \TYP @ \mathit{loc} \\
  \textup{Type Scheme} & \ngTypeScheme & \gramdef &
  \forall_{\overharpoon{\ngLoc^{\ngReg}}}.\;
  \overharpoon{\ngLocatedTy} \ARROW \ngLocatedTy
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-locexpr.tex <==
\[
  \begin{array}{G}
    \textup{Location Expressions} & \ngLE & \gramdef &
      \ngStartRegTy{\ngReg}{\TYP} \\
    & & \gramor & \ngAdvTags{\ngLoc^{\ngPos}}{\DC} \\
    & & \gramor & \ngAfterTy{\ngLocatedTy} \\
    & & \gramor & \ngAdvField{\ngLoc^{\ngPos}}{\DC}{j}{\ngLocatedTy}
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-paths-positions.tex <==
\[
  \begin{array}{G}
    \textup{Field Paths} & \ngPath & \gramdef &
      \ngEmptyPath \gramor \ngFieldKey{\DC}{j}.\ngPath \\
    \textup{Positions} & \ngPos & \gramdef & \ngReg.\ngPath \\
    \textup{Location Atoms} & \ngLoc & \in & \ngAtom \\
    \textup{Locations} & \mathit{loc} & \gramdef & \ngLoc^{\ngPos}
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-program-top.tex <==
\[
  \begin{array}{G}
  \textup{Top-Level Programs} & \mathit{top} & \gramdef &
      \overharpoon{\DD} \;; \overharpoon{\FD} \;; \EXPR
  \end{array}
\]


==> paper-formalism/paper-fragments/gr-termgrammar.tex <==
\[
  \begin{array}{G}
    \textup{Values} & \VAL & \gramdef &
      \var \gramor \ngLocVal{\ngLoc^\ngPos} \\
    \textup{Expressions} & \EXPR & \gramdef & \VAL \\
    & & \gramor & \fapp{\overharpoon{\ngLoc^\ngPos}}{\overharpoon{\VAL}} \\
    & & \gramor & \datacon{\DC}{\ngLoc^\ngPos}{\overharpoon{\VAL}} \\
    & & \gramor & \letpack{\var:\ngLocatedTy}{\EXPR}{\EXPR} \\
    & & \gramor & \letloc{\ngLoc^\ngPos}{\ngLE}{\EXPR} \\
    & & \gramor & \letregty{\ngReg}{\TYP}{\EXPR} \\
    & & \gramor & \case{\VAL}{\overharpoon{\pat}} \\
    \textup{Patterns} & \pat & \gramdef &
      \caseclause{\datacon{\DC}{\!\!}{(\overharpoon{\var:\ngLocatedTy})}}{\EXPR}
  \end{array}
\]


==> tables/pldi/_preamble.tex <==
\providecommand{\gibbondefinecolors}{}
\definecolor{gibbonfast}{RGB}{0,100,0}%
\definecolor{gibbonslow}{RGB}{204,0,0}%
\definecolor{gibbonvanilla}{RGB}{255,243,176}%
\makeatletter
\providecommand{\gibbonvanilla}{}
\@ifpackageloaded{colortbl}{\renewcommand{\gibbonvanilla}{\cellcolor{gibbonvanilla}}}{}
\makeatother
\makeatletter
\@ifundefined{gibbon@fitbox}{\newsavebox{\gibbon@fitbox}}{}
\providecommand{\gibbonfit}[1]{#1}
\renewcommand{\gibbonfit}[1]{%
  \sbox{\gibbon@fitbox}{#1}%
  \ifdim\wd\gibbon@fitbox>\linewidth
    \typeout{GIBBON-TABLE-SCALED: \the\wd\gibbon@fitbox\space into \the\linewidth}%
    \resizebox{\linewidth}{!}{\usebox{\gibbon@fitbox}}%
  \else
    \usebox{\gibbon@fitbox}%
  \fi}
\makeatother

\makeatletter
\providecommand{\gibbonnumfont}{}
\renewcommand{\gibbonnumfont}{%
  \fontsize{\dimexpr\f@size pt+1.5pt\relax}%
          {\dimexpr\f@size pt+3.9pt\relax}\selectfont}
\makeatother



